Invertible Graph Aggregation Can Increase ReLU Readout Width

An invertible graph aggregation preserves the complete feature table, but can increase the size of a classifier that reads one node at a time. For every even $N\ge4$, we construct a labeled tree with $2N$ vertices and maximum degree three. A shared one-hidden-layer rectified linear unit (ReLU) classifier needs one hidden unit on the raw scalar features and exactly $N$ units after one lazy neighborhood mean. All aggregate values are distinct, and the mixing matrix has condition number at most 8. We determine the complete error curve for heads with a free affine term. The width separation persists under scalar perturbations. Under a specified bounded uniform-noise model with one nuisance coordinate, every one-unit aggregate head has expected error at least $1/12$, while a fixed $N$-unit head has zero error. Controlled fits compare trained heads with these explicit feasible scores. On Roman-empire and Tolokers, aggregation improves fitted prediction, and retaining raw features helps at the largest tested parameter budget. Training-only diagnostics include conditional output-layer optimality bounds for eight fixed runs.

==> access-engine-compat.tex <==
% Engine compatibility only; official ieeeaccess.cls and fonts are unchanged.
\RequirePackage{iftex}
\ifXeTeX
  \RequirePackage[T1]{fontenc}
  \makeatletter
  \@namedef{ver@spotcolor.sty}{2026/10/22 local XeTeX compatibility}
  \newcommand\NewSpotColorSpace[1]{}
  \newcommand\AddSpotColor[4]{}
  \newcommand\SetPageColorSpace[1]{}
  \def\SpotSpace{ }
  % Same CMYK alternate specified by the official template for Pantone 3015 C.
  \def\color@spotcolor#1#2{\c@lor@@cmyk1,0.3,0,0.2\@@#1}
  \makeatother
  \AtBeginDocument{%
    % Honor the physical page size declared by the official class.
    \special{papersize=\the\paperwidth,\the\paperheight}%
    \special{pdf:mapfile t1-times.map}%
    \special{pdf:mapfile t1-formata.map}%
    \special{pdf:mapfile t1-giovannistd.map}%
  }
\fi

